Fair and Actionable Causal Prescription Ruleset

Prescriptions, or actionable recommendations, are commonly generated across various fields to influence key outcomes such as improving public health, enhancing economic policies, or increasing business efficiency. While traditional association-based methods may identify correlations, they often fail to reveal the underlying causal factors needed for informed decision-making. On the other hand, in decision-making for tasks with significant societal or economic impact, it is crucial to provide recommendations that are justifiable and equitable in terms of the outcome for both the protected and non-protected groups. Motivated by these two goals, this paper introduces a fairness-aware framework leveraging causal reasoning for generating a set of actionable prescription rules (ruleset) toward betterment of an outcome while preventing exacerbating inequalities for protected groups. By considering group and individual fairness metrics from the literature, we ensure that both protected and non-protected groups benefit from these recommendations, providing a balanced and equitable approach to decision-making. We employ efficient optimizations to explore the vast and complex search space considering both fairness and coverage of the ruleset. Empirical evaluation and case study on real-world datasets demonstrates the utility of our framework for different use cases.

==> 04-complexity.tex <==

\section{Complexity Analysis}
\label{sec:hardness}



% \subsection{Fairness Constraints}
% We study two definitions of fairness from previous literature: statistical parity (SP)~\cite{mehrabi2021survey},  and bounded group loss (BGL)~\cite{agarwal2019fair}. These two definitions are based on equivalent notions of fairness for regression tasks~\cite{agarwal2019fair}. We next provide an extension for these definitions to average treatment effect estimates. 



% \textbf{Group fairness} and \textbf{individual fairness} are two key concepts in the field of algorithmic fairness~\cite{}. Group fairness aims to ensure that different demographic groups receive similar outcomes. For example, in our context, it seeks to ensure that the expected utility for both protected and non-protected groups is similar. In contrast, individual fairness focuses on treating similar individuals similarly, meaning that if two individuals are alike in relevant aspects, they should receive similar outcomes. Both approaches aim to reduce bias and promote fairness. The choice of approach depends on the specific context.
% Next, we present four types of fairness constraints in the context of causal inference: SP and BGL, each of which can be applied to ensure either group or individual fairness.



% % which asks that the prediction be statistically independent of the protected attributes defining the protected group,, which asks that the prediction error restricted to any protected group stay below some pre-determined level. 


% \subsubsection{Statistical parity}
% In SP, the goal is to ensure that the gain in utility of a protected individual is similar to that of any individual from the privileged group.
% We present both group and individual fairness constraints in the context of causal inference. 

% %\sg{To add: what if the rules overlap}
% %\brit{This has already been addressed—each individual is assigned with no more than one rule in practice. If multiple rules are suggested for a person, we assume they choose the worst one.}
% \sg{Need to change to make sure denominator of exp utility is fixed}

% \noindent
% \textbf{Group Fairness}:
% Intuitively, if we sample an individual randomly from the protected group of individuals, the expected increase in outcome (or in other words, utility) should be approximately equal as that of an individual from the unprotected group. This is the same intuition as that of SP for classification.

% Therefore, the SP group fairness constraint is:
% $$|\text{ExpUtility}_p(R) -\text{ExpUtility}_{\bar{p}}(R)| \leq \epsilon$$
% where $\epsilon > 0$ is a threshold. 


% \textbf{Individual Fairness}:
% Intuitively, individual fairness ensures that the expected gain for each protected individual is similar to that for an individual from the privileged group. That means that the expected gain of each rule $r\in R$ on a protected individual should be similar to that of an individual from the privileged group.


% More formally, we define it as:
% For every, $r\in R$,
% $$|utility_p(r) - utility_{\bar{p}}| \leq \epsilon$$

% We can demonstrate that the statistical parity fairness constraint is not a matroid constraint; however, it is a matroid constraint for individual parity. 

% \begin{lemma}
% \label{lemma:sp}
% The statistical parity fairness constraint is not a matroid constraint; however, it is a matroid constraint for individual parity. 
% \end{lemma}
% \begin{proof}
% To show that the statistical parity  fairness constraint is not a matroid, we construct a simple counter example. 

% Consider a dataset $D$ with $50\%$ individuals belonging to the protected group.
% Consider a rule set $R = \{r_1,r_2\}$ such that $coverage(r_1) = \pattern_p$  and  $coverage(r_2) = \pattern_{\bar p}$ and $\text{ExpUtility}_p(r_1) = \text{ExpUtility}_{\bar p}(r_2)  = 100$. This means that the set $R$ is fair. 

% Suppose the statistical parity fairness constraint is a matroid. In that case, any subset of $R$ should also yield a fair prescription. Consider a subset $R' = \{r_2\} \subset R$. 
%  $\text{ExpUtility}_p(r_2) = 0$ and $\text{ExpUtility}_{\bar p}(r_2)  = 100$. Therefore, the $r_2$ alone does not satisfy fairness wrt statistical parity, which is a contradiction.
% \end{proof}


% % \begin{table}[]
% %     \centering
% %  \begin{tabular}{|c|c|c|c|}
% % \hline
% % G & P & T & O \\
% % \hline
% % 1 & 1 & 0 & \$0 \\
% % 1 & 1 & 0 & \$0 \\
% % 1 & 0 & 1 & \$1 \\
% % 1 & 0 & 1 & \$1 \\

% % 0 & 1 & 1 & \$1 \\
% % 0 & 1 & 1 & \$1 \\
% % 0 & 0 & 0 & \$0 \\
% % 0 & 0 & 0 & \$0 \\

% % \hline
% % \end{tabular}
% %     \caption{Example Dataset for Lemma~\ref{lemma:sp}}
% %     \label{tab:sp_ex}
% % \end{table}


% % \begin{proof}[Proof of \cref{lemma:sp}]
% % We show that the hereditary property does not hold, and therefor it follows that this is not a matroid. 

% % Consider a dataset $\db$ with a schema $\attrset = \{G,P, T, O\}$ populated with $2n$ tuples. 
% % For the first $n$ tuples, we assign $t[G] = 1$. In the first half of these tuples we set: $t[P] = 1$, $t[T] = 0$, and $t[O] = 0$, while in the second half, $t[P] = 0$, $t[T] = 1$, and $t[O] = 1$. For the remaining $n$ tuples, the first $\frac{n}{2}$ have $t[P] = 1$, $t[T] = 1$, and $t[O] = 1$, and the rest have $t[P] = 0$, $t[T] = 0$, and $t[O] = 0$.
% % The protected group is defined by the pattern $\pattern_p = \{P = 1\}$, indicating that there are precisely $n$ tuples where $t[P] = 1$. 

% % An illustration of this dataset with 8 tuples is provided in \cref{tab:sp_ex}.


% % Consider the following  prescription rules:
% %     \begin{itemize}
% %         \item \textbf{(A rule that is useful only to non-protected)} $r_1 = (\pattern_g^1, \pattern_t^1)$:, where $\pattern_g^1 = \{G = 1\}$ and $\pattern_t^1 = \{T = 1\}$. We have: $coverage(r_1) =n$, $coverage_p(r_1) = \frac{n}{2}$, $utility_p(r_1) = 0$, and $utility_{\hat{p}}(r_1) = 1$. 
% %         \item  \textbf{(A rule that is useful only to protected)}:  $r_2 =(\pattern_g^2, \pattern_t^2)$, where $\pattern_g^2 = \{G = 0\}$ and $\pattern_t^2 = \{T = 1\}$.
% %         We have: $coverage(r_2) =n$, $coverage_p(r_2) = \frac{n}{2}$, $utility_p(r_2) = 1$, and $utility_{\hat{p}}(r_2) = 0$.
% %     \end{itemize}

% % We get that $overlap(r_1, r_2) = 0$, meaning the rules do not overlap as they pertain to different individuals. Additionally, $r_1$ and $r_2$ cover the entire population.
% % For the rule set $R = {r_1, r_2}$, the statistical parity fairness constraint is met: for a randomly selected protected individual, the expected utility increase is $0.5$ (half get an increase of $1$ and the other half get no increase). Similarly, the expected utility increase for non-protected individuals is also $0.5$. However, when considering any non-empty subset $R'$ of rules from $R$, $R'$ does not satisfy the constraint, as the expected utility for one population will be $0$ and for the other, it will be $0.5$.
% % \end{proof}


% \subsubsection{Bounded group loss (BGL)}: Fair regression with BGL minimizes the overall loss while controlling the worst loss on the protected group~\cite{agarwal2019fair}.
% In our context, this translates to the following fairness constraint: When selecting an individual from the protected group, the outcome increase (utility) should exceed a specified threshold $\tau$.

% \textbf{Group Fairness}: We aim to ensure that the expected utility of a randomly sampled protected individual within $Coverage(R)$ is above a given threshold $\tau$.
% Therefore, the fairness constraint is:
% $$\text{ExpUtility}_p(R) \geq \tau$$

% \textbf{Individual Fairness}: Under individual fairness, we aim to ensure that the gain of every protected individual from $Coverage(R)$ exceeds a threshold $\tau$.
% Therefore, given a threshold $\tau$, we say that a set of rules $R$ satisfies the individual loss constraint if the utility of every rule $r$ on protected individuals is at least $\tau$. More formally, for every rule $r\in R$, $utility_p(r) \geq \tau$.



% Here again, we can demonstrate that the BGL fairness constraint
% is not a matroid constraint; however, it is a matroid constraint for
% individual loss.




% \begin{lemma}
% \label{lem:bgl}
% The BGL fairness constraint is not a matroid, but it is for individual loss.  
% \end{lemma}
% \brit{add proof}

%  \brit{As observed in the example derived from the Stack Overflow datasets. A stricter version, which adheres to matroid properties, requires each rule to guarantee an increase in utility above the specified threshold $\tau$.}
% \begin{proof}

%     \begin{table}[]
%     \centering
%  \begin{tabular}{|c|c|c|c|}
% \hline
% G & P & T & O \\
% \hline
% 1 & 1 & 1 & \$0 \\
% 1 & 1 & 0 & \$0 \\
% 1 & 0 & 0 & \$1 \\
% 1 & 0 & 1 & \$1 \\

% 0 & 1 & 1 & \$1 \\
% 0 & 1 & 0 & \$1 \\
% 0 & 0 & 1 & \$0 \\
% 0 & 0 & 0 & \$0 \\

% \hline
% \end{tabular}
%     \caption{Example Dataset for Lemma~\ref{lemma:bgl}}
%     \label{tab:sp_ex}
% \end{table}

% \end{proof}
% More fairness constraints for regression: Fair Regression: Quantitative Definitions and Reduction-based Algorithms \cite{agarwal2019fair}

 % \textbf{Note:} I am assuming each rule is disjoint, i.e. an individual cannot satisfy multiple rules. For overlapping rules, the equation will change slightly.

 % \brit{the rules are not disjoint, this is too restrictive. For example, one rule can be suggested to people at the age of 25-34, and the second for people from the US. The only restriction is that their coverage should be different (namely, that they are not covering the exact same sub-population). Can you please update the definition? }


% \subsubsection{Individual Fairness}
% We consider two types of individual fairness constraint variants of both group fairness constraints: individual parity ensures that the expected gain of each rule $r\in R$ on a protected individual is similar to that of an individual from the privileged group, and individual loss ensures that the utility of each rule exceeds a threshold $\tau$.

% \paragraph*{Individual Parity.}
% The absolute difference between utility of every rule $r\in R$ over protected individuals is similar to that of a privileged individual. More formally, we define it as:
% For every, $r\in R$,
% $$|utility_p(r) - utility_{\bar{p}}| \leq \epsilon$$
% \begin{lemma}
%     The individual parity fairness constraint is a matroid.
% \end{lemma}
% \sg{need to add proof}


% \paragraph*{Individual Loss.} Given a threshold $\tau$, we say that a set of rules $R$ satisfies the individual loss constraint if  the utility of every rule $r$ on protected individuals is at least $\tau$. More formally, for every rule $r\in R$, $utility_p(r) \geq \tau$.


% \begin{lemma}
%     The individual loss fairness constraint is a matroid.
% \end{lemma}
% \sg{need to add proof}


% \subsection{Coverage Constraints}





We next study the complexity of the \probName\ problem under different constraint combinations. 
First, we demonstrate that the \probName\ problem is an NP-hard problem~\cite{khuller1999budgeted}. Then we show that \probName\ is equivalent to optimizing a non-negative and monotone submodular function. Furthermore, the individual fairness constraint and rule coverage constraints are matroid constraints. Therefore, a greedy approximation algorithm can be used to yield a constant approximation solution.  %Consequently, maximizing it is an NP-hard problem. 

We define the decision version of the \probName\ problem in the following way: Given a bound $k$ on the number of selected rules and a threshold $\tau$ on the expected utility, the question is if there exists a set of at most $k$ rules whose expected utility is at least $\tau$. We can demonstrate that this problem is NP-hard.
\begin{proposition}
\label{prop:unconstrained}
    The \probName\ problem with and without individual fairness constraint is NP-hard.
\end{proposition}



% From \cite{lakkaraju2016interpretable}, we get that $f_1, f_2, f_3$ are non-negative and sub modular. \brit{the utility cant be negative - we consider only positive rules (under the assumption that each one gets no more than one rule).}
We prove that the unconstrained \probName\ problem via a reduction from the max-cover problem. Furthermore, adding individual fairness constraints does not 
We can show that both individual-level fairness constraints (individual parity and individual loss) are matroid constraints. Therefore, adding them does not change the complexity of the problem, as maximizing a non-negative monotone submodular function under a matroid constraint remains NP-hard~\cite{calinescu2007maximizing}.

For the group-level fairness constraints, we can demonstrate that this constraint does not form a matroid and provide a reduction from the Knapsack Problem~\cite{kellerer2004introduction}.

\begin{proposition}
\label{prop:group_fairness}
    \probName\ with a group-fairness constraint is NP-hard
\end{proposition}

% Given a set of $t$ rules $X=\{r_1,\ldots,r_t\}$, we want to identify a subset $S$ such that 




% Let S be a set of all possible rules.

% $$F(S \cup \{r\}) = min\{|F(S)|, |F(S)+f(r)|\}$$


As for coverage constraints, the rule coverage is a matroid constraint (as it can be checked against every rule separately). For the group coverage, on the other hand, we can show that merely finding a solution that satisfies the constraints, even without maximizing expected utility, is NP-hard via a reduction from the Set Cover problem~\cite{feige1998threshold}. 

\begin{proposition}
    \label{prop:group_coverage}
    \probName\ with a group-coverage constraint is NP-hard
\end{proposition}

%A summary of the complexity results is given in \cref{tab:hardness}.

We note that for variants that involve maximizing a submodular function potentially subject to matroid constraints, a greedy approach can yield a solution with approximation guarantees. However, given that the number of potential rules may be quite large (exponential in the database size), we must avoid generating all possible rules to remain efficient. Thus, although our proposed algorithm does not provide theoretical guarantees, it effectively identifies useful sets of rules within a reasonable processing time.



==> abstract.tex <==
Prescriptions, or actionable recommendations, are commonly generated across various fields to influence key outcomes such as improving public health, enhancing economic policies, or increasing business efficiency. While traditional association-based methods may identify correlations, they often fail to reveal the underlying causal factors needed for informed decision-making. On the other hand, in decision making for tasks with significant societal or economic impact, it is crucial to provide recommendations that are interpretable and justifiable, and equitable in terms of the outcome for both the protected and non-protected groups. Motivated by these two goals,  this paper introduces a fairness-aware framework leveraging causal reasoning  for generating a set of interpretable and actionable prescription rules (ruleset) toward betterment of an outcome while preventing exacerbating inequalities for protected groups. By considering group and individual fairness metrics from the literature, we ensure that both protected and non-protected groups benefit from these recommendations, providing a balanced and equitable approach to decision-making. We employ efficient optimizations to explore the vast and complex search space considering both fairness and coverage of the prescription ruleset. Empirical evaluation and case study on real-world datasets 
demonstrates the utility of our framework for different use cases.

==> intro-backup.tex <==
%!TEX root=main.tex

\section{Introduction}
\brit{we shoud discuss causumx, highkit the fitness and not the causal part}

Decision-makers, analysts, data scientists, and policymakers frequently base their conclusions on collected data, using it to extract insights. This allows us to extract actionable recommendations aimed at influencing outcomes of interest, such as increasing product satisfaction or income levels, or decreasing the likelihood of experiencing a serious disease \cite{galhotra2022hyper,lakkaraju2016interpretable}.
Unlike prediction tasks, where achieving high accuracy is the primary goal, decision-making tasks with significant societal impact require recommendations to be actionable, interpretable and justifiable~\cite{}. In these cases, it is essential to provide a clear explanation for why a specific recommendation is made for a particular subpopulation.

Understanding the \emph{causal factors} driving a recommendation aimed at influencing a target outcome for different groups enables informed, data-driven decision-making to address inequities. For example, if a policymaker understands the causal factors affecting the salary of a particular race or gender in a specific country, they can implement corrective measures to improve the situation -- something that may not be achievable using insights based solely on associations. Identifying these causal insights is crucial for addressing societal biases and creating more equitable outcomes.

%a particular race or gender in a specific country, they can implement corrective measures to improve the situation -- something that may not be achievable using insights based solely on associations. 




In this work, we study the problem of generating causal insights (referred to as \emph{prescription rules}), which serve as actionable recommendations to improve an outcome of interest. Causal reasoning is considered as one of the most important requirements,  to generate explanations that are actionable and aligned with human reasoning.
Recent works have introduced causality to the field of database research~\cite{meliou2010causality,  meliou2014causality,salimi2020causal,10.14778/3554821.3554902}. It has been incorporated into various tasks including data discovery~\cite{galhotra2023metam,youngmann2023causal}, query result explanation~\cite{salimi2018bias,youngmann2022explaining,DBLP:journals/pacmmod/YoungmannCGR24}, and large system diagnostics~\cite{markakis2024sawmill,causalsim,sage, gudmundsdottir2017demonstration}. 

\sg{I was not sure so I commented the older version}
%\emph{Causal inference} has been thoroughly studied in AI and Statistics~\cite{pearl2009causal,rubin2005causal}. Causal analysis is a vital tool in determining the effect of a \emph{treatment} on an \emph{outcome}, and has been used in decision-making in medicine \cite{robins2000marginal}, economics \cite{banerjee2011poor}, biology \cite{shipley2016cause}, and in high-stakes areas such as identifying the root causes of failures in critical infrastructure systems to prevent catastrophic outcomes. Recent works have introduced causality to the field of database research~\cite{meliou2010causality,  meliou2014causality,salimi2020causal,10.14778/3554821.3554902}. It has been incorporated into various tasks including data discovery~\cite{galhotra2023metam,youngmann2023causal}, query result explanation~\cite{salimi2018bias,youngmann2022explaining,DBLP:journals/pacmmod/YoungmannCGR24}, and large system diagnostics~\cite{markakis2024sawmill,causalsim,sage, gudmundsdottir2017demonstration}. We propose leveraging causal inference to generate interpretable and justifiable insights (referred to as \emph{prescription rules}), which serve as actionable recommendations to improve an outcome of interest. Causal reasoning is considered as one of the most important requirements,  to generate insights that are actionable and aligned with human reasoning.


Next, we introduce a running example that will be referenced throughout the paper.




\begin{table*}[]
\footnotesize
    \centering
    	\caption{\textnormal{A subset of the Stack Overflow dataset.}}
         \label{tab:data}
    	% \vspace{-4mm}
  			\begin{tabular}[b]{|l|l|l|c|l|l|c|l|c|}
  			
				%\multicolumn{9}{c}{\textbf{Users}}\\ 
				\hline

				\textbf{ID}
    
    % \textbf{Country}& \textbf{Continent} 
    
    &\textbf{Gender} &\textbf{Ethnicity}&
				\textbf{Age} &\textbf{Role} &
				\textbf{Education} &\textbf{Country}&\textbf{Undergrad Major}&\textbf{Salary}
				\\ \hline

				1 &Male&White&26&Data Scientist & PhD& US&Computer Science&180k\\
    		2 &Non-binary&White&32&QA developer & Bachelor's degree& US&Mechanical Eng.&83k\\

 3 &Male&South Asian&29&C-suite executive  & Bachelor's degree & India&Computer Science&24k\\

  4 &Female&South Asian&25&Back-end developer  & Master's degree & India&Mathematics&7.5k\\

  5 &Male&East Asian&21&Back-end developer & Bachelor's degree & China&Computer Science&19k\\
  

        % $\ldots$ &  $\ldots$&  $\ldots$&  $\ldots$&  $\ldots$&  $\ldots$&  $\ldots$&  $\ldots$&  $\ldots$&  $\ldots$&  $\ldots$\\
    \hline
			\end{tabular}
\end{table*}




\begin{example}	%
Consider the Stack Overflow (SO) annual developer survey
\cite{stackoverflowreport}, where respondents from around the world answer
questions about their jobs and demographics. A sample of the dataset with a subset of the
attributes is presented in \cref{tab:data}.

Alex, a researcher in the UN finance department, is interested in discovering ways to increase the salaries of high-tech employees worldwide. She is looking for a set of actionable recommendations (referred to as \emph{prescription rules}) to raise the overall average salary.

Using association-based approaches~\cite{chen2018optimization,lakkaraju2016interpretable}, she may find that individuals who spend fewer than 5 hours a day on their computer have higher salaries than those who work more hours. However, this insight merely highlights a correlation: C-level executives, for instance, often spend more time in meetings and, therefore, less time at their computers. Naturally, their higher salaries are due to their position, not the amount of time they spend on their computer.

\brit{Benton, please change this part according to the experiments}
In contrast, through causal analysis, she discovers that for individuals aged 20-30 in the U.S., holding a PhD can result in a \$2,000 annual salary increase, while for those over 40 worldwide, learning Python can boost their salary by \$3,000 per year.
\sg{Discuss how rules can be unfair here}
\end{example}


Our objective is to generate a small set of prescription rules aimed at increasing (or decreasing) an outcome of interest. This is framed as an optimization problem where the goal is to select the fewest prescription rules that maximize utility (i.e., the expected increase or decrease in the outcome). However, focusing solely on maximizing utility can result in a scenario where only a small fraction of the population gets significant improvement, while others experience no benefit. Additionally, even if a large portion of the population receives recommendations, a protected subpopulation might not share the benefits and, worse, their situation could deteriorate, exacerbating inequalities.

We, therefore, enable users to incorporate various \emph{coverage and fairness constraints} along with the overall objective. Following research concerning fairness in database research~\cite{stoyanovich2020responsible,galhotra2022causal}, we assume the existence of a protected subpopulation, defined by sensitive attributes such as gender, or ethnicity. Coverage constraints ensure that a substantial fraction of the population and protected subpopulation receive at least one recommendation. Fairness constraint ensure that the expected utility of the protected population is ``comparable'' compared to the utility received by the unprotected individuals. We devise novel group and individual fairness definitions tailored for prescription rules. 

\begin{example}
    \brit{TODO: add an example to show how fairness and coverage constraints affect the solution}
\end{example}


\noindent
Our main contributions are as follows. \\
%\begin{itemize}[leftmargin=*,topsep=0pt]
{\bf (1)} We {\bf develop a framework that generates a set of prescription rules to enhance an outcome of interest.} A prescription rule consists of a \emph{grouping pattern} and a \emph{treatment pattern}, representing the target subpopulation and the actionable recommendation for that group, respectively. The strength of the causal effect of this treatment on the subgroup is used to measure the expected utility of a rule. Our objective is to identify the smallest set of prescription rules that maximizes overall expected utility. We refer to this problem as the \probName\ problem, and show that it is NP-hard.
    \par
    \noindent
{\bf (2)} We {\bf develop several coverage and fairness constraints} to ensure that the solution for the \probName\ problem is applied to a sufficient number of individuals and to minimize inequalities. We establish various definitions for coverage and fairness constraints tailored for causal analysis and analyze the complexity of the \probName\ problem subject to different constraints.  
    \par
    \noindent
{\bf (3)} We {\bf propose a general three-step algorithmic framework named \sysName}. The first step involves mining frequent grouping patterns using the Apriori algorithm~\cite{agrawal1994fast}. In the second step, we employ a lattice-based algorithm to find promising treatment patterns for each grouping pattern identified in the previous step. Finally, the third step applies a greedy approach to determine a solution. \sysName\ can be easily adapted to accommodate all variants of the \probName\ problem.
\par
\noindent
{\bf (4)} We provide a thorough {\bf experimental analysis} and {\bf multiple case study} that include two datasets, four baselines, and 18 variations of our problem with different constraints. \brit{TODO} 
%\end{itemize}


\paragraph*{Paper outline} Related work is discussed in \cref{sec:related}. Background on causal inference is provided in \Cref{sec:prelim}, and our problem formulation can be found in \cref{sec:problem}. Complexity analysis of the problem studied under different constraints is given in \cref{sec:hardness}, followed by a discussion on selecting the appropriate problem variant. Our algorithmic framework is presented in \cref{sec:algo}, a case study demonstrating the impact of different constraint configurations on the solution is given in \cref{exp:problem_variants}, and our experimental evaluation is detailed in \cref{sec:experiments}. Finally, we discuss the limitations of our framework in \cref{sec:conc}.

% \noindent
% \boxed{\parbox{\columnwidth}{$\bullet$ 
% For people with a professional degree, move to the United Kingdom
%  (coverage = 435 (20), coverage-protected = 20 (13), utility = 186855, utility-protected = 0.)\\
% $\bullet$ For graphic developers, move to the	United States
%  (coverage = 116 (29), coverage-protected = 8 (2), utility = 169431, utility-protected = 0).\\
% $\bullet$ For people who have no formal education, move to the United States
%  (coverage = 123 (34), coverage-protected = 7 (2), utility = 206742, utility-protected = 0).\\
% % \textcolor{red}{size = 38, length = 76, overlap = 64029181, utility = 1659307}\\
% \textcolor{blue}{overall coverage =674, expected utility = 187485
% coverage-protected = 35, expected utility-protected = 0}
% \sr{should mention protected group, and possibly not mention coverage in the intro or just intuitively like high coverage}
% }}


% Alex notes that although these rules result in a \$187,485 increase in the overall salary for those to whom they apply, they only affect a small fraction of the population, specifically 674 individuals. Additionally, although the expected salary increase is substantial, there is no expected increase in salary for non-males, a subpopulation of particular interest to Alex. In other words, applying these rules would result in no gain for non-males.
% \end{example}

% \begin{example}[Episode 2 - coverage and fairness constraints]
% Alex introduces coverage and fairness constraints to ensure that enough people will benefit from the rules and that they will be \emph{fair} with respect to non-males. Specifically, she demands that the benefit for a randomly chosen individual to whom one of the rules applies is nearly the same as the benefit for a randomly chosen individual who identifies as non-male and to whom one of the rules applies.

% After adding these constraints, \sysName\ recommends the following set of prescription rules:



% \noindent
% \boxed{\parbox{\columnwidth}{$\bullet$ 
% For people who have no formal education, move to the United States
%  (coverage = 123 (34), coverage-protected = 7 (2), utility = 206742, utility-protected = 0)\\
% $\bullet$ 
% For females, change role to	DevOps specialist (coverage = 2256 (47), coverage-protected = 2256 (47), utility = 90023, utility-protected = 90023).\\
% $\bullet$ For people with a Master's degree, move to the	United States
%  (coverage = 9097 (2222), coverage-protected = 642 (236), utility = 85390, utility-protected = 84201).\\
% % \textcolor{red}{size = 38, length = 76, overlap = 64029181, utility = 1659307}\\
% \textcolor{blue}{overall coverage =11476	
% , expected utility = 87601,
% coverage-protected = 2905, expected utility-protected = 88519}
% }} 







% \begin{figure}[t]
%         \centering
%         \begin{minipage}[b]{1.0\linewidth}
%             \small
%             \begin{tcolorbox}[colback=white]
%             \vspace{-2mm}
% $\bullet$ For backend developers, the treatment with the highest effect on salary is “Country = US” effect size = 78646
% \begin{itemize}
%     \item For non-male the effect is only: 59429
%     \item For male the effect is 80454
% \end{itemize}

% $\bullet$ For frontend developers, the treatment with the highest effect is :Formal Education = Bachelor's degree” effect size: 17340
% \begin{itemize}
%     \item For white the effect is 33464
%     \item For non-white the effect is 15320
% \end{itemize}


% $\bullet$ For people in Europe, the treatment with the highest effect on salary is “DevType = C-suite executive” effect size = 53254
% \begin{itemize}
%     \item For white the effect is 55112
%     \item For non-white 35249
% \end{itemize}



%             \vspace{-2mm}
%             \end{tcolorbox}
%         \end{minipage}%%
%          % \vspace{-4mm}
%         \caption{Set of prescription rules.}
%         \label{fig:so-explanation}
%     \end{figure}


==> old-ilp.tex <==


\begin{figure}
    \centering
    \small
    %\begin{footnotesize}
    \begin{tcolorbox}[colback=white]
    \vspace{-2mm}
    \begin{equation*}
    \begin{aligned}
   & \max \quad \underbrace{\left(\sum_{j = 1}^l g_j \cdot w_j\right)}_{\text{utility objective}}  + \underbrace{\left (l - \sum_{j = 1}^l g_j \right )}_{\text{ size objective }}  \quad   
   % + \underbrace{\left (m\cdot l^2 - \sum_{i = 1}^m\sum_{j = 1}^l t_{i,j} \cdot g_j \right )}_{\text{ overlap objective }}\quad 
    \textrm{s.t.} \\
    % (1)~\sum_{j = 1}^l g_j \leq k, \quad \\
    &  (1)~t_i {\leq} \sum_{j{:} T_i {\in} \pattern_j} g_j ~\forall i = 1 \text{ to }m, ~p_i {\leq} \sum_{j{:} T_i {\in} \pattern_j} g_j ~\forall i = 1 \text{ to }m_p    \\
     & (2) \text{ group coverage: } ~\sum_{i = 1}^m t_i \geq \theta_1 \cdot m, ~\sum_{i = 1}^{m_p} p_i \geq \theta_2 \cdot m_p\quad \\
     & (3) \text{ (SP) group fairness: } \\
     &\left | \left ( \frac{1}{m_p}\sum_{i}^{m_p} \min_{g_j | g_j = 1} (p_{i,j} {\cdot} g_j {\cdot} w_{j,p}) \right ) {-} \left ( \frac{1}{m}\sum_{i}^{m} \max_{g_j | g_j {=} 1} (t_{i,j} {\cdot} g_j {\cdot} w_{j}) \right )  \right | {\leq} \epsilon\\
      % & (3^2) \text{ BGL group fairness constraint} \left | \left ( \frac{1}{m_p}\sum_{i}^{m_p} \min_{g_j | g_j = 1} (p_{i,j} \cdot g_j \cdot w_{j,p}) \right )  \right | \geq \epsilon\\
     & (4)~t_i, p_h, g_j \in \{0, 1\} ~\forall i = 1 \text{ to }m, ~\forall h = 1 \text{ to } m_p, ~\forall j = 1 \text{ to }l \\
    \end{aligned}
    % }
    \end{equation*}
    \vspace{-2mm}
    \end{tcolorbox}
    %\end{footnotesize}  
    \vspace{-1mm}
    \caption{Example ILP formulation with group coverage and SP group fairness constraints.} 
    \label{fig:lp}
\end{figure}


==> response.tex <==
\twocolumn
\section*{Response Letter for Submission 1379 (Shepherd Submission 1621)}

%\noindent \textbf{Dear reviewers,}

\noindent 
We would like to express our gratitude to the reviewers for their valuable feedback.
In response to the reviewers' comments and according to the revision plan, we focused on addressing four main areas of improvement: (1) improving the experimental analysis, (2) enhancing the presentation, (3) extending the discussion on related works, and (4) clarifying our limitations.
To address these issues, we have provided a detailed explanation of our responses to the concerns that were raised by all reviewers. We have also addressed each reviewer's comments individually.

Updates made in response to specific comments are highlighted in the revised manuscript using the following colors:
\begin{itemize}
\item \common{Changes for multiple reviewers in Orange}
\item \reva{Reviewer 1 in Green}
\item \revb{Reviewer 2 in Magenta}
\item \revc{Reviewer 3 in Purple} 
\end{itemize}



\subsection*{Summary of the Main Changes}
We provide a brief overview of the main changes we made. \blue{Reviewer\#1, \#2, and \#4 are referred to as R1, R2, and R3 respectively.}



% \vspace{1mm}
\noindent
% {\bf{(\colorbox{pink}{Point \textrm{1}}) Additional Experiments}}. 
\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{1}})
% \label{rev:point-1}
Improving the experimental analysis}} Based on the reviewers' suggestions, we enhanced the experimental evaluation in the following ways:


$\bullet$ \textbf{Comparison with baselines}: We expanded the comparison with the baselines (FRL~\cite{chen2018optimization} and IDS~\cite{lakkaraju2016interpretable}) to include quantitative metrics, including the solution size, coverage, accuracy, and execution time \blue{(addressing R2.O1)}.

\lastday{We would like to clarify that the rules generated by IDS and FRL baselines are prediction rules (e.g., IF owning a house = YES, THEN credit score = 1). We note that, as such, {\bf these rules generated by IDS and FRL do not provide any intervention to improve outcomes and do not include any grouping patterns}. To compare IDS and FRL with our approach, we  developed two variants of these two approaches: (i) considered the IF clause of these rules as grouping patterns and used Step 2  (\cref{subsec:treatment_patterns}) of our algorithm to determine the relevant treatment for each grouping pattern.  (ii) considered the IF clause of each rule as a treatment pattern where the grouping pattern is the whole population. }


% Specifically, (1) we have added more details about the rules generated by IDS and FRL in {\bf \cref{tab:problem_variants}}, now including the solution size and their coverage. 
% To compare the expected utility, we proceed as follows: The rules generated by these baselines are prediction rules (e.g., IF owning a house = YES, THEN credit score = 1). We note that, as such, {\bf these rules generated by IDS and FRL do not provide any intervention to improve outcomes and do not include any grouping patterns}. We, therefore, treat the IF clauses as the selected grouping patterns and then apply step 2 (\cref{subsec:treatment_patterns}) of our algorithm to determine the relevant treatment for each grouping pattern. For the resulting set of prescription rules, we report the expected utility for both protected and non-protected groups. \red{This process can be viewed as an alternative method for generating grouping patterns}.


\lastday{For these two variants, we report the solution size, coverage, expected utility for protected and non-protected, and the unfairness
The results are presented in 
{\bf \cref{tab:problem_variants}}. Notably, the expected utility for both protected and non-protected groups across both datasets is generally lower than that achieved by \sysName.  \sysName\ consistently delivers higher expected utility for both groups and a smaller difference between these values. This indicates that our approach to mining grouping and intervention patterns is more effective than relying on these algorithms for the same purpose.  However, we note (and also mention in the paper) that the rules in IDS and FRL had different objectives (prediction accuracy) and have been evaluated differently for quantitative comparison using our metrics (as was asked by the reviewers).}



(2) Additionally, we updated {\bf \cref{exp:scalability} (Figure~\ref{fig:runtime_dataset_size} and Figure~\ref{fig:runtime_attributes})} to include a runtime analysis for the baselines as well, examining how their runtime varies with the number of tuples and attributes. The running time of \sysName and the baselines (IDS and FRL) is comparable (\textbf{\Cref{fig:runtime_dataset_size}}). 
\lastday{FRL is an order of magnitude slower than IDS because it uses a Bayesian modeling approach to simultaneously select a subset of rules and determine their optimal permutation, which involves solving a computationally intensive combinatorial problem. In contrast, IDS leverages submodular optimization on an unordered set of rules, significantly reducing the complexity of the search.}
We also compared the running time on varying the number of mutable and immutable attributes (\textbf{\Cref{fig:runtime_attributes}}). FRL and IDS do not distinguish between mutable and immutable attributes, and their running time depends on the total number of attributes, as with more attributes the search space of possible rules increases. 

$\bullet$ \textbf{Protected groups}: We provided a more detailed explanation of the protected groups analyzed and the rationale behind their selection \blue{(addressing R2.O2)}. Specifically, we now explain in {\bf Section \ref{sec:casestudy}} that the protected groups were selected to represent subgroups where the desired outcome was relatively low and that they are sufficiently large to ensure the discovery of statistically significant rules. The protected group in the Stack Overflow data is defined as individuals from countries with a low GDP (using the GDP attribute, which is categorical in this dataset). This group constitutes 21.5\% of the data. In the German Credit data, the protected group is defined as single females, and this group constitutes 9.2\% of the data. 
% \red{{\bf **REVISIT**}} 
    



\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{2}})
\label{rev:point-1}
Enhancing the presentation}} To enhance the paper's presentation, we have made the following revisions.



$\bullet$ \textbf{Usability}: We provided an explanation of how the proposed framework may potentially be used by policymakers \blue{(addressing R1.O1)}. Specifically, we now discuss an example scenario in {\bf Section \ref{sec:conc}} that the policymaker selects the target outcome and the relevant problem variant (e.g., imposing coverage and/or fairness constraints). The system then generates a prescription ruleset for the policymaker to implement. The framework assumes that the policymaker will publish the relevant recommendations for each subpopulation. However, if not all rules are provided to the users, disparities among subpopulations may increase, and a study of proper and fair usage of rules suggested by our framework remains a future work.
  

$\bullet$ \textbf{Usage of LLMs}: 
As \blue{R1.O7} pointed out, the generated rules mostly follow a template, and we do not need LLMs to translate the rules to natural language sentences. In the revised paper, we replaced the explanations with a template version to present them without relying on LLMs, to avoid hallucinations and errors.

%We will clarify our use of LLMs and revise the prompts to ensure it does not introduce errors.  We utilized ChatGPT to translate prescription rules into natural language. Each rule included the following components: grouping pattern, intervention pattern, overall coverage, coverage for protected groups, and overall, protected, and non-protected expected utility. ChatGPT was prompted to rephrase these elements into a natural language sentence.  To minimize the risk of hallucination, we will refine our prompts by using precise templates. This approach ensures the content remains unchanged, with ChatGPT solely rephrasing the rule into a sentence without altering the numbers or meaning (addressing R1.O7).


$\bullet$ \textbf{Presentation of Result Summary}: We adjusted the colored boxes to make their content easier to read and present the results summary in a more accessible format  \blue{(addressing R1.O8)}. \lastday{We also removed the results summary discussion, now pointing out our main findings in the text.} Please refer to the revised {\bf Section \ref{sec:casestudy}}.

$\bullet$ \textbf{Patterns \& WHERE clauses}: We clarified in {\bf Section \ref{subsec:rules}} the relation between WHERE clause and a pattern \blue{(addressing R3.O1)}. Specifically, we now mention that \emph{patterns} is a commonly used notation in query result explanation research~\cite{roy2014formal,wu2013scorpion,el2014interpretable,lin2021detecting}. Generally, patterns are equivalent to the WHERE clause in SQL queries. However, in this work, we focus on a specific type of pattern: a conjunction of predicates, as has been done in prior query result explanation research~\cite{roy2014formal,wu2013scorpion,el2014interpretable,lin2021detecting,DBLP:journals/pacmmod/YoungmannCGR24}.

$\bullet$ \textbf{Motivating example}: We have revised {\bf the introduction} to make it more concrete by rephrasing it to include more realistic and practical examples \blue{(addressing R3.O2)}. Specifically, we focused on the two use cases examined in our experimental evaluation: increasing the average salary of high-tech employees and improving the average credit risk score. 

Additionally, \blue{to address R1.O2 and interactive discussion with R1}, we revised the motivating example of the Stack Overflow dataset ({\bf \cref{example:ex1} and \cref{ex:intro_example_3}}) to avoid relying on the (unconvincing) causal relationship between exercising and salary. A similar revision was made in the case study presented in {\bf Section \ref{sec:casestudy}}.

$\bullet$ \textbf{Typos}: We have thoroughly proofread the paper and the code repository to eliminate any typos or errors \blue{(addressing multiple comments by the reviewers  R1.11, R1.12, R2.12, R3.10)}.




\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{3}})
% \label{rev:point-1}
Extending the discussion on related works}} 
 To the best of our knowledge, no existing framework generates causal-based, fairness-aware actionable recommendations. However, we expanded our discussion of {\bf related work (Section~\ref{sec:related})} from relevant conferences to include recent literature on alternative definitions of fairness (e.g.,\cite{jain2024algorithmic, somerstep2024algorithmic}) and causal-based resource allocation approaches (e.g., \cite{majumdar2024carma, ehyaei2023robustness}) \blue{(addressing R1.O6, R1.O3)}. We emphasized that this work focuses on four definitions of fairness -- statistical parity and bounded group loss, considering both individual and group fairness -- as an initial step. Exploring additional definitions of fairness is an interesting direction for future research.  
 %
 We have fixed reference \cite{zehlike2022fairness} and \cite{zehlike2022fairness2}  as mentioned in \blue{R2.12}.




\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{4}})
Clarifying our
limitations. }} 
Based on the reviewers' comments, we extended the discussion on the limitations of the proposed framework in the following ways:

$\bullet$ \textbf{Causal DAG quality}: In the revised {\bf Section \ref{sec:conc}}, we clarified that the generated rules can be influenced by several factors, including the quality of the input causal DAG \blue{(addressing R1.O2)}. Specifically, we acknowledge that inaccuracies in the DAG may lead to flawed rules. Consequently, we assume that the causal DAG is provided as part of the input, with the responsibility for validating its correctness resting on the policymaker. Nonetheless, the causal DAG only needs to specify causal dependencies between variables without detailing the nature of those dependencies.



To examine the quality of the causal DAG on the performance, we also added an experiment evaluating the robustness of our method when the causal graph is noisy.
Specifically, in the revised {\bf Section \ref{subsec:causal_DAG_robustness}}, we examine the impact of different causal DAGs on the rules. The causal DAGs considered are as follows: 
\textbf{(1) 1-layer Indep DAG:} A causal DAG where all attributes are independent of each other and only impact the outcome. This setting is similar to the scenario where the causal DAG is ignored.
\textbf{(2) 2-layer Mutable DAG:} A simplified DAG where immutable attributes affect the mutable attributes, which impact the outcome variable. In this DAG, all immutable attributes act as confounders but do not directly impact the outcome.
%Another default causal DAG where all immutable attributes point to mutable attributes, which in turn point to the outcome.  
\textbf{(3) 2-layer DAG:} A simplified DAG where all variables affect the outcome but the mutable attributes are also confounded by all immutable attributes (i.e., we add direct edges from immutable attributes to the outcome in the previous 2-layer mutable DAG). 
%Another 2-layer causal DAG. In this DAG, to include confounding variables, all edges in the default-2-layer DAG are present, with additional edges from the top layer to the outcome.  
\textbf{(4) PC DAG:} A causal DAG generated by the PC causal discovery algorithm~\cite{spirtes2001causation}.

\lastday{The results are depicted in \textbf{\cref{tab:causal_dag_variants}}. We report the expected utility as computed over the different causal DAGs. We observe that the expected utility remains similar for the Stack overflow dataset, demonstrating robustness towards the choice of causal dag. The results show some variability in German credit. However, the PC DAG and the original causal DAG are the most accurate (as they are based on the data distribution and domain knowledge) and achieve the highest coverage and expected utility.}
%\brit{TODO} \red{ADD ONE MORE 2 -LAYER?}



Lastly, we clarified that the example dataset (\textbf{\cref{tab:data}}) and the example causal DAG (\textbf{\cref{fig:causal_DAG}}) represent only a subset of the data, consisting of 20 variables.  


% In our running example from Stack Overflow, the \verb|Exercise| variable (indicating how many times per week an individual exercises) has a directed causal path to the \verb|HoursComputer| variable (indicating how many hours per day an individual works on a computer), which in turn directly affects the \verb|Salary| variable. Thus, based on this DAG, exercising has an indirect causal effect on salary.  

    


$\bullet$ \textbf{Theoretical guarantees}: We acknowledge that our algorithm does not provide formal guarantees for approximating the \probName\ problem \blue{(addressing R1.O4)}, and we clarified this in the revised {\bf Section \ref{sec:algo}}. As expected, the problem is NP-hard in simple settings (proofs deferred to the full version due to lack of space) and even developing good heuristics considering several parameters and constraints is non-trivial. However, we emphasize that each selected rule represents an intervention that is statistically significant. Specifically, based on causal analysis, the expected utility reflects the anticipated average increase in the outcome for the specific subpopulation to which the rule applies. Nevertheless, as we mention in the revised {\bf Section \ref{sec:conc}}, the quality of the generated rules may be influenced by several factors, including data quality, the correctness of the input causal DAG, and the method used to estimate causal effects. 
%\red{MENTION ROBUSTNESS HERE?}

 
 $\bullet$ \textbf{Explainability}: Another limitation we now address in the revised paper pertains to the explainability and interpretability of the generated rules \blue{(addressing R3.O3, and the interactive discussion with R1)}.
 %While if-then rules are generally considered interpretable by humans~\cite{lakkaraju2016interpretable,guidotti2018local,van2021evaluating,pradhan2022interpretable,chen2018optimization}, 
 While if-then rules for prediction or causation mined from data are considered explainable or interpretable in the literature \cite{lakkaraju2016interpretable,pradhan2022interpretable,van2021evaluating,guidotti2018local,chen2018optimization}, we note that no additional explanations or justifications come with the prescriptive rules mined by \sysName, which may be added in future work. 
%However, as mentioned in Point 4, the rules themselves are considered explainable or interpretable in the literature [1-5]. We will clarify this in the paper.
%We also note that prescription rules consist of conjunctions of predicates, which may not always be explainable. 
Generating meaningful explanations to describe how the treatment patterns impact the outcome and the variability of the outcome within various sub-populations are deferred to future work. This is now discussed in {\bf Section~\ref{sec:conc}.}
 \cut{
 \red{prescription rules consist of conjunctions of predicates, which may not always be explainable.} For instance, in a highly detailed dataset, a possible rule might suggest that {\em individuals aged between 18.5 and 21.2 years should learn programming in Python}. Understanding the rationale behind such a rule is not straightforward. A potential direction for future work involves binning continuous variables into semantically meaningful ranges while ensuring that sound causal inference can still be performed on the binned data. We clarified this issue in the revised 
{\bf Section \ref{sec:conc}}
}.



\vspace{4mm}
\noindent
%This concludes the summary of the main revisions we plan to make.
Below, we give responses to the meta-reviewer's and reviewers' comments and refer to the above points for details to avoid repetition.\\


\subsection*{Meta-Review}
\vspace{1mm}
\noindent
\emph{\blue{The authors consider the task of mining from a table a set of rules that can be turned into recommendations that are fair in the sense that there is not too large of a difference in expected outcome between a protected and a non-protected group.\\
%
The reviewers request a deeper consideration of the fairness literature, to better position the results, including in the evaluation (R2.01) as well as addressing the points below.}}\\
\noindent
\emph{\blue{{\bf 5. Required Changes}\\
R1 01-08\\
R2.01/02\\
R2: 01-O2\\
}}
\textbf{Ans}. We thank the meta-reviewer and the reviewers for the revision opportunity. As discussed in the summary above and in the responses below, we addressed all required changes and other comments in the revised paper.\\

\subsection*{Reviewer \#1}
\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O1}}
\emph{\blue{The general framework of how this work could be used is unclear.
If at least some individuals do not hear about the recommendation, they would clearly be at a disadvantage. Conversely, if the rules are known "internally", e.g., the bank has its internal rules on who gets credit, people who know the rules play the game better than the others. This is already the case today. Clearly, the authors take a step forward by considering protected subgroups, I understand that they seek to make things more fair. But how their proposed rules can be leveraged to that purpose is unclear.
Moreover, in general, most resources are finite, e.g., total salary to pay to the developers, or credit to be given out by a bank.
If all the groups followed the recommendations, would everyone's salary really increase? Would all customers be awarded credit? Or are rules/criteria in real life used to divide a finite resource, with a more or less arbitrary threshold drawn somewhere?}} 
\textbf{Ans}. We thank the reviewer for highlighting these issues. Our work is one of the initial works in this area, and the questions asked by the reviewers are important future work. As noted in {\bf Point 2} above, we included a discussion on the intended usability of the system and the potential risks of improper use in the revised {\bf Section \ref{sec:conc}}. Additionally, we now mention in the revised Section \ref{sec:conc} that future work would focus on extending our framework to include additional constraints related to available resources.

In addition to whether the rules are conveyed fairly to the targeted individual, another question is whether 
%The reviewer raises an interesting point about ensuring that 
the generated rules cover all individuals. The coverage constraint in this work intends to enforce such a requirement. However, not all applications necessitate universal coverage. For instance, a political party may implement targeted policies to maximize votes, or a company might offer incentives to individuals more likely to purchase a product. Our framework provides the flexibility to specify these coverage requirements while maintaining fairness with respect to sensitive attributes. However, an in-depth study of the proper and fair usage of the rules suggested by this system remains a future work.

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O2}} \emph{\blue{The authors' notion of causality is hard to understand in some places (examples).
The authors state in many places that their approach is causal, not correlation-based. Yet it takes a leap of faith to assume that exercising X days a week causally improves one's salary, especially for young people (considering that the bad effects of lack of exercise start showing in one's 40s or 50s).
Also, exercise does not appear at all in Table 1; nor does it appear in the partial DAG (Figure 1), nor is there some substitute attribute or anything related to the exercise aspect.
In my view, these "exercise impacts salary" examples are not helping the paper to be convincing.}} 
\textbf{Ans}. We agree with the reviewer on this point. Following the reviewer's suggestion, we replaced our running example and presented rules for the stack overflow dataset to avoid relying on the (unconvincing) causal relationship between exercising and salary (as mentioned in {\bf Point 2} above, see {\bf \cref{example:ex1} and \cref{ex:intro_example_3}}). Table 1 and Figure 1 show only a subset of the attributes.

Please also refer to our discussion in {\bf Point 4} regarding the quality of the input causal DAG. 

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O3}} \emph{\blue{Other aspects of fairness deserve more discussion.
The example given early on states that a certain rule whcih would improve salaries by 13000\$ for protected people and 44000\$ for everyone. Whether or not this is acceptable/desirable depends on the local purchase power and who the group consists of (does a majority of users live in India? or in the US? the calculations would not be the same). Maybe this is part of the authors' future work (mentioned at the end) of the paper.}} 
\textbf{Ans}.
The reviewer has raised an interesting point about varied purchasing power and cost of living in different countries. One way to address this would be to modify the objective function to maximize the ratio of salary and purchasing power. However, principled techniques to address these issues are indeed interesting directions for future work, and we discuss this in {\bf Section~\ref{sec:conc}}.
Please also see {\bf Point 3} for discussions on fairness definitions.
%We have discussed this limitation in more detail in the future work section. %\brit{to discuss}
%In the revised paper, we will provide additional details about the distributions in the examined datasets to give more context for the generated rules. As noted in Point 3 above, we also plan to expand our discussion of other definitions of fairness in the related work section.

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O4}} \emph{\blue{As the authors acknowledge, there are no formal guarantee of the quality of their obtained rules.}} 
\textbf{Ans}. Please refer to our answer in {\bf Point 4} above (see {\bf Section \ref{sec:algo} and Section~\ref{sec:conc}}). 

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O5}} \emph{\blue{How many among the "Result Summary" statements required some experiments to establish, vs. some that can be analytically shown or exhibited with small examples?}} 
\textbf{Ans}. 
%We agree with the reviewer on this point. 
To fit additional material, we decided to remove the result summary since the individual experiments discuss the findings. 
\cut{
Some statements in the results summary, such as the observation that fairness often comes at the cost of overall expected utility, are straightforward and intuitive. We revised the discussion in the results summary to emphasize the more interesting and novel findings uncovered through our analysis. Please refer to the revised {\bf \Cref{sec:casestudy}}.  
}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O6}} \emph{\blue{The paper is welcome at SIGMOD where fairness is one of the topics. However, it would be good if the authors did a more comprehensive comparison with the stazte of the art in FAccT and also RecSys, to ensure: has their problem never been looked at? It would be good to make sure.}} 
\textbf{Ans}. Thank you. In our revised related work ({\bf \cref{sec:related}}), we have discussed additional related work, including previous work on rule mining~\cite{lakkaraju2016interpretable,lawless2023interpretable}, causal rule mining~\cite{DBLP:journals/pacmmod/YoungmannCGR24} and fair causal analysis~\cite{plecko2022causal,plecko2023causal,zhang2022adaptive} techniques. We also discuss alternative fairness definition~\cite{binns2020apparent,garcia2021maxmin,DBLP:journals/pacmmod/ZhangTPCW23,somerstep2024algorithmic,smith2022recsys,ekstrand2019fairness,gao2020counteracting} and fairness of
allocated resources~\cite{majumdar2024carma, ehyaei2023robustness}. Some of these new references appeared in FAccT and RecSys. We could not find previous works that consider both causal rule mining and fairness aspects. Please also refer to our response in {\bf Point 3} above. 





\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O7}} \emph{\blue{Why use ChatGPT to generate very simple, template-like text (out of patterns), especially considering that it may hallucinate and introduce errors?}} 
\textbf{Ans} Please see our response in {\bf Point 2} above. We now do not use ChatGPT to rephrase the rules and use a fixed template.


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O8}} \emph{\blue{It is OK to show sample rules as "figures" with smaller font, but it's a pity to do so for important content such as the Result Summary.}} 
\textbf{Ans}. Thank you for this comment. We revised the presentation to ensure the main findings of the results are clear and more accessible. As mentioned under R1.O5, we have removed the result summary and results are now discussed along with the experiments. 


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.11 and R1.12}} \emph{\blue{Availability and Minor Remarks.}} \textbf{Ans}. Thank you for highlighting these issues. We addressed them all, and thoroughly proofread the paper and the repository.

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{Additional Comments from Interactive Discussions}}

% \cut{
% \emph{\blue{
% (1) Thank you for your revision plan! In Point 4, you state: "Exercise variable (indicating how many times per week an individual exercises) has a directed causal path to the HoursComputer variable (indicating how many hours per day an individual works on a computer), which in turn directly affects the Salary variable."
% A. Can you please clarify: increasing Exercise leads to which effet on HoursComputer? (increase or decrease?)
% B. From the paper's statement: "male students should exercise 3-4 times per week, and pursue an undergraduate major in CS. This can boost their salary by \$25,578 per year", I understand that the (increase or decrease) in HoursComputer leads to an increase in Salary. Is this correct?
% If (as your answer to Point 4 seems to state) the authors are not very confident in the A. or B. causal paths, the data may not be of very good quality, the example may be confuse readers. It would then be better to replace it. What do you think?}} 
% }

%  %We had more clarifications about this question in the feedback discussion, which we could not include due to space constraints. 
% \cut{Thank you for asking this question. First, we clarify the answers:

% A. Increasing exercise may have a causal effect on HoursComputer, but it can be either way. Increased exercise time (heavily) may decrease the time to work at the computer, but it can also increase the time to work making a person more fit, The advantage of using a causal DAG is that we only need to know a causal dependency exists without specifying or quantifying the nature of causal effect, i.e., we do not need to fit a model for the causal effect or decide whether the effect is increasing or decreasing when we use a causal DAG.

% B. The causal rule returned by our framework is only as stated, i.e., it does not advise whether the exercise time should be increased or decreased from the current status. It only states that the treatment pattern "HoursExercise = 3-4 AND MAjor = CS" has a positive CATE of \$25,578 on male student population.

% We will look for better examples, also clarify what the causal rules imply, how the causal DAG is used, and that the actual nature of causal dependencies (increase/decrease, measure) is not needed in our framework.

% Thanks,
% authors
% }

% \vspace{1mm}
% \noindent
% \cut{
% \emph{\blue{
% (2) Thank you for clarifying. I understand that your approach does not need to establish in which direction a parameter affects another, e.g., whether exercise increases or decreases HoursComputer.
% I believe the Explainability paragraph in Point 4 of your revision plan also states this, i.e., there is no explanation or justification that comes with the prescription, and it is not really explainable.
% While the work is interesting, the wording "prescription", "recommendation", or "causal", bothers me, because it is hard to imagine outputs of this algorithm being recommended to actual humans
% without some causal reasoning/explanation attached.
% In the example we discussed, "that we only need to know a causal dependency exists without specifying or quantifying the nature of causal effect" perhaps simplifies things computationally.
% However, the causal/logical links not sought after ("those that we don't need to know") are probably those that would convince someone to adopt the "prescriptions".}}
% }
% %

% \emph{\blue{
% \ldots{} At this point, I think we agree that:\\
% - a better example would be less puzzling\\
% - the limitations you propose in Point 4. of the revision plan are very helpful to clarify what the approach can (and cannot) provide}}
% \cut{Thanks a lot again, for asking us the questions and this engaging discussion. We agree with the reviewer on the final two points and will address them in the revision:
% 1. A better example would be less puzzling
% 2. The limitations proposed in Point 4. of the revision plan will be clarified as a discussion of what our approach can (and cannot) provide.

% We would like to further clarify and confirm a few other things mentioned by the reviewer:

% A. There is indeed no *additional* explanation or justification that comes with the prescription. However, as mentioned in Point 4, the rules themselves are considered explainable or interpretable in the literature [1-5]. We will clarify this in the paper.

% B. The *causal* aspect of this work is based on the vast causal inference literature on observational causal studies in Statistics and AI on observed or collected data. Under certain assumptions (that are known to be untestable), causal claims can be made from collected or observed data, and Average Treatment Effect (ATE) and Conditional Average Treatment Effect (CATE) on a subpopulation can be estimated. We follow Judea Pearl’s Graphical Causal Model from the AI literature [6] and use the DoWhy package released by Microsoft (https://github.com/py-why/dowhy) to estimate ATE and CATE. Indeed, the estimation of ATE and CATE depends on the quality of the causal DAG as mentioned in Point 4 of the revision plan, which we assume is given as background information. The causal DAG only needs causal dependencies between variables without specifying its nature. In the revision, we will vary the causal DAGs to evaluate the dependency of our framework on the accuracy of the causal DAG.

% C. Causal analysis is the main foundation for any *prescription* or *recommendation* beyond predictions. When possible, one would do a randomized controlled trial (e.g., when a new vaccine is tested), but often they are not possible due to cost/ethics/feasibility issues, and one depends on observational causal study (used in sociology, econometrics, psychology). Indeed, observational causal study depends on assumptions (ignorability, causal DAG) that may not hold in a scenario, but that still a causal claim. This was the reason we used the terms prescription and recommendation. However, we agree that one should know the assumptions and limitations of these claims, and we will make sure to clarify this in the revised paper and explain the rationale behind using the terms causal and prescription along with their limitations.

% We will be happy to answer if the reviewer has a follow-up question or comment.
% Many thanks for the discussion and the thoughtful comments,
% the authors

% [1] Guidotti, Riccardo, et al. "Local rule-based explanations of black box decision systems." arXiv preprint arXiv:1805.10820 (2018).
% [2] van der Waa, Jasper, et al. "Evaluating XAI: A comparison of rule-based and example-based explanations." Artificial intelligence 291 (2021): 103404.
% [3] Pradhan, Romila, et al. "Interpretable data-based explanations for fairness debugging." Proceedings of the 2022 International Conference on Management of Data. 2022.
% [4] Lakkaraju, Himabindu, Stephen H. Bach, and Jure Leskovec. "Interpretable decision sets: A joint framework for description and prediction." Proceedings of the 22nd ACM SIGKDD international conference on knowledge discovery and data mining. 2016.
% [5] Chaofan Chen and Cynthia Rudin. 2018. An optimization approach to learning
% falling rule lists. In International conference on artificial intelligence and statistics.
% PMLR, 604–612.
% [6] Pearl, Judea. Causality. Cambridge university press, 2009.
% }
% \cut{\emph{\blue{
% %(3) Thank you for the more extensive explanation. 
% \ldots{} I believe it will be helpful to clarify the notions of causality and explainability you use early on,
% to avoid confusions and guide the readers. This, and an example readers can more easily interpret, will help the paper reach its potential!
% }}}
\textbf{Ans}. Thank you for taking the time to discuss with us in the interactive discussion forum. 
\begin{itemize}
    \item As mentioned under R1.O2, we have replaced the exercise example with a more convincing example. The example of exercise and our follow-up discussion about this will be added to the full version.
\item We have discussed in detail in {\bf Section \ref{sec:conc}} several limitations of our current framework and directions for future work, including the limitations pointed out by the reviewers.
\item As discussed under {\bf Point 4}, we have added experiments varying the causal DAG to evaluate the robustness of our approach in terms of the causal DAGs. Please see revised {\bf Section \ref{subsec:causal_DAG_robustness}}.
\item We have added a discussion on the explainability and prescriptive nature of the rules in {\bf Section~\ref{sec:conc}} as a concluding remark. 
\end{itemize}



\subsection*{Reviewer \#2}
\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.O1}} \emph{ \blue{The experimental comparison with state-of-the-art solutions is currently limited and should be improved.
The comparison with the baselines is performed only at the qualitative level (Section 7.2). This analysis should also be extended at the quantitative level, comparing the solutions in terms of size, coverage, fairness metrics, and execution time. A more complete evaluation would prove the effectiveness of the results.}} 
\textbf{Ans}. We have revised our experiments following the suggestion. Please see our response to {\bf Point 1} above. 

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.O2}} \emph{ \blue{The paper states that, in the experiments, ‘the protected groups were selected to represent subgroups where the desired outcome was relatively low and sufficiently large (approximately 30\% of the population) to ensure the discovery of statistically significant rules.’ I find this indication unclear. Which are the protected groups? I invite the authors to clearly specify it.}} 
\textbf{Ans}. Please see our response in {\bf Point 1} above. 



\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.12}} \emph{\blue{-How were the three rules shown in the example selected? What are the criteria?
Moreover, it would be interesting to discuss the overall rules.
- Table 5 compares the solutions also in terms of size, coverage, and expected utility as Table 4. I suggest extending the caption.
-Typos
Survey [97] has a peer-review published version}} \textbf{Ans}. 
We have added the following discussion in {\bf \Cref{sec:casestudy}}. We chose the rules by picking one randomly from each category (one that favors the protected group, one that favors the non-protected, and another that is more balanced). We also mention that the full lists of rules are available in \cite{fullversion}.
Thank you for pointing out the typos, the caption of Table 5, and reference [97] (now~\cite{zehlike2022fairness}). We fixed them and proofread the paper.

\subsection*{Reviewer \#3}
\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.O1}} \emph{ \blue{Why call this a pattern? This is a WHERE clause, and the following discussion of coverage is selectivity. Why create new jargon?}} 
\textbf{Ans}. Please see our response in {\bf Point 2} above. 

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.O2}} \emph{  \blue{The verbiage in the abstract and introduction - presecriptions are for change - both personal health and organization... very motherhood and apple pie, but difficult to map directly to this work. Could we bring it down from such lofty goals? Given the high-level that the introduction is written at, it is unclear what a realistic prescription could be. A clear, complete and well motivated running example, tied into the introduction that can then be used to clearly explain components of the paper - such as the granularity of a prescription, or algorithmic results later - would do well.}} 
\textbf{Ans}. We thank the reviewer for this comment. As mentioned in {\bf Point 2} above, we revised the introduction to focus
on the two use cases examined in our experimental evaluation:
increasing the average salary of high-tech employees and improving
the average credit risk score. 


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.O3}} \emph{ \blue{There is a statement about understanding and explanability in the motivation. However, the explainability component is not clearly described in teh approach or evaluation. This either needs to be removed, or strengthened.}} 
\textbf{Ans}. We agree with the reviewer on this point. We removed these statements from the paper and included a discussion on enhancing explainability in {\bf \Cref{sec:conc}}. Please refer to our response in {\bf Point 4} above.

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.10}} \textbf{Ans}. \emph{\blue{Honestly, the formatting with the callout boxes bothers me a bit. I can't tell if I'm just being old, or if there is a readability problem here}}
\textbf{Ans}. Thank you for pointing this out. We revised the formatting of the boxes. 



==> revision_plan.tex <==
\twocolumn
\section*{Revision plan of Submission 1379 (Shepherd Submission 1621)}
\noindent \textbf{Dear reviewers,}

\noindent 
We would like to express our gratitude to the reviewers for their valuable feedback.
In response to the reviewers' comments, we will focus on addressing four main areas of improvement: (1) improving the experimental analysis, (2) enhancing the presentation, (3) extending the discussion on related works, and (4) clarifying our limitations.
To address these issues, we have provided a detailed explanation of our responses to the main concerns that were raised by all reviewers. We have also addressed each reviewer's comments individually.




\subsection*{Summary of the Revision Plan}
We provide a brief overview of the main changes we plan to implement in the revision. \blue{Reviewer\#1, \#2, and \#4 are referred to as R1, R2, and R3 respectively.}



% \vspace{1mm}
\noindent
% {\bf{(\colorbox{pink}{Point \textrm{1}}) Additional Experiments}}. 
\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{1}})
% \label{rev:point-1}
Improving the experimental analysis}} Based on the reviewers' suggestions, we plan to enhance the experimental evaluation in the following ways:


$\bullet$ \textbf{Comparison with baselines}: We will expand the comparison with the baselines (FRL and IDS) to include quantitative metrics, including the solution size, coverage, fairness measures, and execution time \blue{(addressing R2.O1)}.

$\bullet$ \textbf{Protected groups}: We will provide a more detailed explanation of the protected groups analyzed and the rationale behind selecting them \blue{(addressing R2.O2)}.
    



\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{2}})
\label{rev:point-1}
Enhancing the presentation}} To enhance the paper's presentation, we plan to make the following revisions:



$\bullet$ \textbf{Usability}: We will provide a clear explanation of how the proposed framework is intended for use by policymakers \blue{(addressing R1.O1)}. Specifically, the policymaker selects the target outcome and the relevant problem variant (e.g., imposing coverage and/or fairness constraints). The system then generates a prescription ruleset for the policymaker to implement. The framework assumes that the policymaker will publish the relevant recommendations to each subpopulation. However, if not all rules are provided to the users, disparities among subpopulations may increase.  
We will highlight this limitation of our framework and include a discussion on its intended usability in the revised paper.   

$\bullet$ \textbf{Usage of LLMs}: 
We utilized ChatGPT to translate prescription rules into natural language. This translation was done to make the rules easy to understand. However, as \blue{R1.O7} pointed out, the explanations mostly follow a template, and we do not need GPT for this task. We will replace current explanations with a template version to present them without using ChatGPT.

%We will clarify our use of LLMs and revise the prompts to ensure it does not introduce errors.  We utilized ChatGPT to translate prescription rules into natural language. Each rule included the following components: grouping pattern, intervention pattern, overall coverage, coverage for protected groups, and overall, protected, and non-protected expected utility. ChatGPT was prompted to rephrase these elements into a natural language sentence.  To minimize the risk of hallucination, we will refine our prompts by using precise templates. This approach ensures the content remains unchanged, with ChatGPT solely rephrasing the rule into a sentence without altering the numbers or meaning (addressing R1.O7).


$\bullet$ \textbf{Presentation of Result Summary}: We will adjust the colored boxes to make their content easier to read (increasing the fonts and changing the colors) and present the results summary in a more accessible format, avoiding the use of colored boxes for the results summary discussion \blue{(addressing R1.O8)}.

$\bullet$ \textbf{Patterns \& WHERE clauses}: We will clarify the relation between WHERE clause and a pattern \blue{(addressing R3.O1)}. Specifically, we will clarify that \emph{patterns} is a commonly used notation in query result explanation research~\cite{roy2014formal,wu2013scorpion,el2014interpretable,lin2021detecting}. Generally, patterns are equivalent to the WHERE clause in SQL queries. However, in this work, we focus on a specific type of pattern: a conjunction of predicates, as has been done in prior query result explanation research~\cite{roy2014formal,wu2013scorpion,el2014interpretable,lin2021detecting,DBLP:journals/pacmmod/YoungmannCGR24}.

$\bullet$ \textbf{Motivating example}: We will revise the introduction to make it more concrete by rephrasing it to include more realistic and practical examples \blue{(addressing R3.O2)}. Specifically, we will focus on the two use cases examined in our experimental evaluation: increasing the average salary of high-tech employees and improving the average credit risk score.

$\bullet$ \textbf{Typos}: We will thoroughly proofread the paper and the code repository to eliminate any typos or errors \blue{(addressing multiple comments by the reviewers  R1.11, R1.12, R2.12, R3.10)}.




\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{3}})
% \label{rev:point-1}
Extending the discussion on related works}}

 To the best of our knowledge, no existing framework generates causal-based, fairness-aware actionable recommendations. However, we will broaden our discussion of related work from relevant conferences to include recent literature on alternative definitions of fairness (e.g., \cite{jain2024algorithmic, somerstep2024algorithmic}) and causal-based resource allocation approaches (e.g., \cite{majumdar2024carma, ehyaei2023robustness}) \blue{(addressing R1.O6, R1.O3)}. We will emphasize that this work focuses on four definitions of fairness -- statistical parity and bounded group loss, considering both individual and group fairness -- as an initial step. Exploring additional definitions of fairness is an interesting direction for future research.  We will fix reference [97] as mentioned in \blue{R2.12}.




\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{4}})
Clarifying our
limitations. }} 
Based on the reviewers' comments, we plan to extend the discussion on the limitations of the proposed framework in the following ways:

$\bullet$ \textbf{Causal DAG quality}: We will clarify that the generated rules may be influenced by various factors, including the quality of the input causal DAG \blue{(addressing R1.O2)}. We will also add an experiment evaluating the robustness of our method when the causal graph is noisy. The example dataset (\cref{tab:data}) and the example causal DAG (\cref{fig:causal_DAG}) represent only a subset of the data, consisting of 20 variables.  
In our running example from Stack Overflow, the \verb|Exercise| variable (indicating how many times per week an individual exercises) has a directed causal path to the \verb|HoursComputer| variable (indicating how many hours per day an individual works on a computer), which in turn directly affects the \verb|Salary| variable. Thus, based on this DAG, exercising has an indirect causal effect on salary.  
The causal DAG was constructed using the causal discovery algorithm proposed in \cite{youngmann2023causal}. We acknowledge that inaccuracies in the DAG may result in flawed rules. Therefore, we assume the causal DAG is provided as part of the input and will emphasize that it is the policymaker's responsibility to validate the correctness of the causal DAG.
    


$\bullet$ \textbf{Theoretical guarantees}: We acknowledge that our algorithm does not provide formal guarantees for approximating the \probName\ problem \blue{(addressing R1.O4)}, and we will clarify this further in the revised paper. As expected, the problem is NP-hard in simple settings and even developing a good heuristics considering several parameters and constraints was non-trivial. However, we emphasize that each selected rule represents an intervention that is statistically significant. Specifically, based on causal analysis, the expected utility reflects the anticipated average increase in the outcome for the specific subpopulation to which the rule applies. Nevertheless, as we mention in Section \ref{sec:conc}, the quality of the generated rules may be influenced by several factors, including data quality, the correctness of the input causal DAG, and the method used to estimate causal effects. We will add approximations and further theoretical analysis as future work.

 
 $\bullet$ \textbf{Explainability}: Another limitation we will address in the revised paper pertains to the explainability and interpretability of the generated rules \blue{(addressing R3.O3)}. While if-then rules are generally considered interpretable by humans~\cite{lakkaraju2016interpretable}, prescription rules consist of conjunctions of predicates, which may not always be explainable. For instance, in a highly detailed dataset, a possible rule might suggest that individuals aged between 18.5 and 21.2 years should learn programming in Python. Understanding the rationale behind such a rule is not straightforward. A potential direction for future work involves binning continuous variables into semantically meaningful ranges while ensuring that sound causal inference can still be performed on the binned data. We will clarify this in the revised paper.



\vspace{4mm}
This concludes the summary of the main revisions we plan to make.
Below, you will find detailed responses to the reviewers' comments.\\


\subsection*{Meta-Review}
\vspace{1mm}
\noindent
\emph{\blue{The authors consider the task of mining from a table a set of rules that can be turned into recommendations that are fair in the sense that there is not too large of a difference in expected outcome between a protected and a non-protected group.\\
%
The reviewers request a deeper consideration of the fairness literature, to better position the results, including in the evaluation (R2.01) as well as addressing the points below.}}\\
\noindent
\emph{\blue{{\bf 5. Required Changes}\\
R1 01-08\\
R2.01/02\\
R2: 01-O2\\
}}
\textbf{Ans}. We thank the meta-reviewer and the reviewers for the revision opportunity. As discussed in the summary above and in the responses below, we will address all required changes and other comments in the revised paper.\\

\subsection*{Reviewer \#1}
\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O1}}
\emph{\blue{The general framework of how this work could be used is unclear.
If at least some individuals do not hear about the recommendation, they would clearly be at a disadvantage. Conversely, if the rules are known "internally", e.g., the bank has its internal rules on who gets credit, people who know the rules play the game better than the others. This is already the case today. Clearly, the authors take a step forward by considering protected subgroups, I understand that they seek to make things more fair. But how their proposed rules can be leveraged to that purpose is unclear.
Moreover, in general, most resources are finite, e.g., total salary to pay to the developers, or credit to be given out by a bank.
If all the groups followed the recommendations, would everyone's salary really increase? Would all customers be awarded credit? Or are rules/criteria in real life used to divide a finite resource, with a more or less arbitrary threshold drawn somewhere?}} 
\textbf{Ans}. We thank the reviewer for highlighting this important issue. As noted in Point 2 above, we plan to include a discussion on the intended usability of the system and the potential risks of improper use. Additionally, we will provide a detailed discussion of additional constraints related to available resources and outline these as potential extensions for future work.

The reviewer raises an interesting point about ensuring that rules cover all individuals. To address this, we include a coverage constraint that allows for the enforcement of such a requirement. However, not all applications necessitate universal coverage. For instance, a political party may implement targeted policies to maximize votes, or a company might offer incentives to individuals more likely to purchase a product. Our framework provides the flexibility to specify these coverage requirements while maintaining fairness with respect to sensitive attributes.

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O2}} \emph{\blue{The authors' notion of causality is hard to understand in some places (examples).
The authors state in many places that their approach is causal, not correlation-based. Yet it takes a leap of faith to assume that exercising X days a week causally improves one's salary, especially for young people (considering that the bad effects of lack of exercise start showing in one's 40s or 50s).
Also, exercise does not appear at all in Table 1; nor does it appear in the partial DAG (Figure 1), nor is there some substitute attribute or anything related to the exercise aspect.
In my view, these "exercise impacts salary" examples are not helping the paper to be convincing.}} 
\textbf{Ans}. Please refer to our response in point 4 above, discussing the causal DAG quality.  

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O3}} \emph{\blue{Other aspects of fairness deserve more discussion.
The example given early on states that a certain rule whcih would improve salaries by 13000\$ for protected people and 44000\$ for everyone. Whether or not this is acceptable/desirable depends on the local purchase power and who the group consists of (does a majority of users live in India? or in the US? the calculations would not be the same). Maybe this is part of the authors' future work (mentioned at the end) of the paper.}} 
\textbf{Ans}.
The reviewer has raised an interesting point about varied purchasing power and cost of living in different countries. A potential way to fix this would be to modify the objective function. However, principled techniques to address these issues is part of future work.
We will discuss this limitation in more detail in the future work section.
%In the revised paper, we will provide additional details about the distributions in the examined datasets to give more context for the generated rules. As noted in Point 3 above, we also plan to expand our discussion of other definitions of fairness in the related work section.

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O4}} \emph{\blue{As the authors acknowledge, there are no formal guarantee of the quality of their obtained rules.}} 
\textbf{Ans}. Please refer to our answer in Point 4 above. 

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O5}} \emph{\blue{How many among the "Result Summary" statements required some experiments to establish, vs. some that can be analytically shown or exhibited with small examples?}} 
\textbf{Ans}. We agree with the reviewer on this point. Some statements in the results summary, such as the observation that fairness often comes at the cost of overall expected utility, are straightforward and intuitive. We will revise the discussion in the results summary to emphasize the more interesting and novel findings uncovered through our analysis.  


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O6}} \emph{\blue{The paper is welcome at SIGMOD where fairness is one of the topics. However, it would be good if the authors did a more comprehensive comparison with the stazte of the art in FAccT and also RecSys, to ensure: has their problem never been looked at? It would be good to make sure.}} 
\textbf{Ans}. Please refer to our response in Point 3 above. 


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O7}} \emph{\blue{Why use ChatGPT to generate very simple, template-like text (out of patterns), especially considering that it may hallucinate and introduce errors?}} 
\textbf{Ans}. Please see our response in Point 2 above. 


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.O8}} \emph{\blue{It is OK to show sample rules as "figures" with smaller font, but it's a pity to do so for important content such as the Result Summary.}} 
\textbf{Ans}. Thank you for this comment. We will revise the presentation to ensure the main findings of the results are clearer and more accessible. Please refer to our response for R1.O5. 


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.11 and R1.12}} \emph{\blue{Availability and Minor Remarks.}} \textbf{Ans}. Thank you for highlighting these issues. We will address them, thoroughly proofread the paper, and review the repository.


\subsection*{Reviewer \#2}
\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.O1}} \emph{ \blue{The experimental comparison with state-of-the-art solutions is currently limited and should be improved.
The comparison with the baselines is performed only at the qualitative level (Section 7.2). This analysis should also be extended at the quantitative level, comparing the solutions in terms of size, coverage, fairness metrics, and execution time. A more complete evaluation would prove the effectiveness of the results.}} 
\textbf{Ans}. Please see our response to Point 1 above. 

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.O2}} \emph{ \blue{The paper states that, in the experiments, ‘the protected groups were selected to represent subgroups where the desired outcome was relatively low and sufficiently large (approximately 30\% of the population) to ensure the discovery of statistically significant rules.’ I find this indication unclear. Which are the protected groups? I invite the authors to clearly specify it.}} 
\textbf{Ans}. Please see our response in Point 1 above. 



\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.12}} \emph{\blue{-How were the three rules shown in the example selected? What are the criteria?
Moreover, it would be interesting to discuss the overall rules.
- Table 5 compares the solutions also in terms of size, coverage, and expected utility as Table 4. I suggest extending the caption.
-Typos
Survey [97] has a peer-review published version}} \textbf{Ans}. 
We chose the rules by picking one randomly from each category (one which favors the protected group, one which favors the non-protected and another one that is more balanced). We will discuss all rules for the example as well.
Thank you for pointing out the typos, the caption of Table 5, and reference [97]. We will fix these and proofread the paper.

\subsection*{Reviewer \#3}
\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.O1}} \emph{ \blue{Why call this a pattern? This is a WHERE clause, and the following discussion of coverage is selectivity. Why create new jargon?}} 
\textbf{Ans}. Please see our response in Point 2 above. 

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.O2}} \emph{  \blue{The verbiage in the abstract and introduction - presecriptions are for change - both personal health and organization... very motherhood and apple pie, but difficult to map directly to this work. Could we bring it down from such lofty goals? Given the high-level that the introduction is written at, it is unclear what a realistic prescription could be. A clear, complete and well motivated running example, tied into the introduction that can then be used to clearly explain components of the paper - such as the granularity of a prescription, or algorithmic results later - would do well.}} 
\textbf{Ans}. We thank the reviewer for this comment. As mentioned in Point 2 above, we will revise the introduction to focus
on the two use cases examined in our experimental evaluation:
increasing the average salary of high-tech employees and improving
the average credit risk score. 


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.O3}} \emph{ \blue{There is a statement about understanding and explanability in the motivation. However, the explainability component is not clearly described in teh approach or evaluation. This either needs to be removed, or strengthened.}} 
\textbf{Ans}. We agree with the reviewer on this point. We will remove these statements from the paper and include a discussion on enhancing explainability in the future work section. Please refer to our response in Point 4 above.

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.10}} \textbf{Ans}. \emph{\blue{Honestly, the formatting with the callout boxes bothers me a bit. I can't tell if I'm just being old, or if there is a readability problem here}}
Thank you for pointing this out. We will revise the formatting of the callout boxes. 



==> saved-conc.tex <==
%\vspace{-3mm}
\section{Limitations and Future Work}
\label{sec:conc}


\sysName\ generates actionable, causal-based recommendations to improve a target outcome while incorporating coverage and fairness constraints. \common{To the best of our knowledge, this is one of the first works in this direction, and several directions of future work remain. In this section, we discuss some of the current limitations of \sysName\ and future directions. }
\reva{

{\bf Generation and usage of rules by \sysName.~} \sysName\ can be used to recommend actions for different subpopulations toward optimizing a target. As an example scenario, a policymaker may select the target outcome and the parameters for coverage and fairness constraint (which may be iteratively varied and inspected based on the application).
%the relevant problem variant (e.g., coverage and fairness constraints). 
\sysName\ then generates a prescription ruleset as recommended actions for different subpopulations.
%for the policymaker to implement. 
The current framework assumes that the policymaker is trustworthy, will not misuse the rules, and will publish the relevant recommendations for each subpopulation. However, it is important to note that if not all rules are provided to all subpopulations, disparities among subpopulations may increase. Further, the generated rules do not consider global constraints, e.g., if the targeted outcome is salary in an institution, there may be a total budget, and the rules may not be applicable independently. Other variants of the problem remain future work.}

{\bf Considering constraints and resources.~} We acknowledge that the generated rules may lack robustness, meaning they might not impact all individuals receiving the recommendation in the same way. An exciting direction for future research would be to focus on ensuring the robustness of prescription rules. Another direction for future work is to account for the cost of interventions. Some interventions may be impractical (e.g., pursuing a bachelor’s degree in CS for someone who already holds a PhD in CS) or vary significantly in cost (e.g., moving to the US versus learning Python). \reva{Additionally, the gain in objective may vary across different subpopulations. For example, increase in $\$10000$ revenue would have caried impact on quality of life in different countries, depending on the cost of living and purchasing power. } Future research will incorporate intervention costs to generate budget-constrained prescription rules \reva{as well as address finite resource allocation scenarios to account for cases where the population size that can achieve improved outcomes is limited}.

{\bf Extension to multi-table data.~} \sysName\ currently supports a single-relation database without dependencies among tuples to ensure compliance with the SUTVA assumption~\cite{rubin2005causal} (discussed in \cref{sec:background-causal}). However, this assumption breaks down even in single-table databases with tuple dependencies. In single-table settings, intervention and grouping patterns are straightforward to define. Extending these definitions to multi-table databases, where grouping attributes and interventions may originate from different tables, introduces a significant challenge. This complexity arises due to many-to-many relationships and cross-table patterns. 
Previous work, such as \cite{salimi2020causal,galhotra2022hyper}, has extended causal models to handle multi-table data, but they have not explicitly targeted recommendations for subgroups. Expanding our framework to support multi-relational databases with complex dependencies remains an important direction for future research. Notably, prior work leveraging causal inference \cite{ma2023xinsight, youngmann2022explaining, salimi2018bias, DBLP:journals/pacmmod/YoungmannCGR24} has also primarily focused on single-table settings.





\revc{We also note that prescription rules consist of conjunctions of predicates, which may not always be explainable. For instance, in a highly detailed dataset, a possible rule might suggest that individuals aged 18.5- 21.2 should learn Python. Understanding the rationale behind such a rule is not straightforward. Future work would focus on binning continuous variables into meaningful ranges while preserving causal inference validity. }


Finally, it is essential to recognize that the generated rules may be influenced by several factors, including the method used to evaluate causal effects, the thresholds set for the constraints, the overall quality of the data, and the quality of the causal DAG.
\reva{Specifically, we acknowledge that inaccuracies in the DAG may lead to flawed rules. Consequently, we assume that the causal DAG is provided as part of the input, with the responsibility for validating its correctness resting on the policymaker. Nonetheless, the causal DAG only needs to specify causal dependencies between variables without detailing the nature of those dependencies.}




==> vary-coverage-table.tex <==
\begin{table*}[h!]
\centering
\small
\caption{Comparison of Solutions in Terms of Coverage}
\label{tab:problem_variants}
\begin{tabular}{lccccccc}
\toprule
\textbf{Stack Overflow (SP fairness)} & \textbf{\# rules} & \textbf{coverage} & \textbf{coverage pro} & \textbf{exp utility} & \textbf{exp utility non-pro}&\textbf{exp utility pro} &\textbf{unfairness} \\
\midrule 
Rule coverage (25\%) & 18& 100.0\%& 100.0\%& 23941.72& 24012.45& 16607.88& 7404.57 \\
Rule coverage (50\%) &6& 99.99\%& 99.99\%& 21350.47& 21305.46& 16604.92& 4700.54 \\
Rule coverage (75\%)  & 2& 97.79\%& 99.17\%& 17841.33& 17771.65& 17882.83& -111.18\\
Rule coverage (90\%)  & 2& 97.79\%& 99.17\%& 17841.33& 17771.65& 17882.83& -111.18 \\
Group coverage (25\%)  & 20& 99.89\%& 99.9\%& 32620.47& 32616.56& 18144.23& 14472.33 \\
Group coverage (50\%) & 20& 99.88\%& 99.94\%& 32592.89& 32566.25& 17712.47& 14853.78 \\
Group coverage (75\%) & 20& 99.71\%& 99.93\%& 32618.08& 32585.24& 15308.97& 17276.27\\
Group coverage (90\%) & 20& 99.66\%& 99.91\%& 32444.38& 32396.22& 18043.07& 14353.15\\
        
\midrule
\textbf{German Credit (BGL fairness)} & \textbf{\# rules} & \textbf{coverage} & \textbf{coverage pro} & \textbf{exp utility} & \textbf{exp utility non-pro}&\textbf{exp utility pro}&\textbf{unfariness}   \\
\midrule 
Rule coverage (25\%) & 7& 96.40\%& 100.0\%& 0.31& 0.31& 0.28& 0.03 \\
Rule coverage (50\%) &1& 84.5\%& 97.83\%& 0.27& 0.26& 0.31& -0.05 \\
Rule coverage (75\%)  & 1& 84.5\%& 97.83\%& 0.27& 0.26& 0.31& -0.05\\
Rule coverage (90\%)  & 0& 0\%& 0\%& 0.0& 0.0& 0.0& 0.0 \\
Group coverage (25\%)  & 14& 100.0\%& 100.0\%& 0.39& 0.39& 0.31& 0.08 \\
Group coverage (50\%) & 17& 100.0\%& 100.0\%& 0.39& 0.39& 0.3& 0.09 \\
Group coverage (75\%) & 16& 100.0\%& 100.0\%& 0.39& 0.39& 0.28& 0.11\\
Group coverage (90\%) & 18& 100.0\%& 100.0\%& 0.39& 0.39& 0.3& 0.09\\
\bottomrule
\end{tabular}
\end{table*}

